21 cm observations: calibration, strategies, observables

This chapter aims to provide a review of the basics of 21 cm interferometric observations and its methodologies. A summary of the main concepts of radio interferometry and their connection with the 21 cm observables - power spectra and images - is presented. I then provide a review of interferometric calibration and its interplay with foreground separation, including the current open challenges in calibration of 21 cm observations. Finally, a review of 21 cm instrument designs in the light of calibration choices and observing strategies follows.

==> compile_pdflatex <==
pdflatex ms
bibtex Furlanetto/chapter
bibtex Mirocha/chapter
bibtex Greig/chapter
bibtex Bernardi/chapter
bibtex Chapman_Jelic/chapter
bibtex Greenhill_Subrahmanyan/chapter
bibtex Trott_Pober/chapter
bibtex Koopmans_Bernardi/chapter
pdflatex ms
pdflatex ms
rm *~ *.aux *.log *.blg *.out *\#
